Positivity-preserving third order DG schemes for Poisson--Nernst--Planck equations

In this paper, we design and analyze third order positivity-preserving discontinuous Galerkin (DG) schemes for solving the time-dependent system of Poisson--Nernst--Planck (PNP) equations, which has found much use in diverse applications. Our DG method with Euler forward time discretization is shown to preserve the positivity of cell averages at all time steps. The positivity of numerical solutions is then restored by a scaling limiter in reference to positive weighted cell averages. The method is also shown to preserve steady states. Numerical examples are presented to demonstrate the third order accuracy and illustrate the positivity-preserving property in both one and two dimensions.

==> deleted_from_old_intro.tex <==

To illustrate the construction for (i) we take the drift-diffusion equation as a model,   
\begin{align}\label{fp}
  \partial_t c  = \nabla \cdot(\nabla c+  c \nabla \psi),
  \end{align}
and reformulate it as 
 \begin{align}\label{fp+}
 \partial_t c  =\nabla \cdot \left( M \nabla g \right), \quad  c  =g M, \quad M=e^{-\psi}.
   \end{align}
This reformulation or its variant has been explored in \cite{DWZ20, HP19, HH20, LW20a, LW20b,LY14b} in their design of positive schemes by the finite difference method. Here we apply the direct discontinuous Galerkin (DDG) spatial discretization to (\ref{fp+}). The main feature of the DDG method, as originally introduced in \cite{LY09, LY10}, lies in the numerical flux choices for the solution gradient, which involve higher order derivatives evaluated across cell interfaces. For the DDG method with the reformulation (\ref{fp+}), the cell average of $c$ can no longer be updated directly from that in the previous time step, yet the propagation is kept well by a projection step which relates the weighted average of $g$ to the cell average of $c$. We show that the results obtained in \cite{LY14b} can be extended to the case when the potential is governed by the Poisson equation, as in (\ref{mc}).
To fulfill the objective (i), we consult \cite{ LY14b}  where authors designed up to third order DDG method that satisfies a strict maximum principle for the Fokker-Planck (FP) equation
\begin{subequations}
\begin{align}\label{fp}
  &\partial_t f  = \nabla \cdot(\nabla f+  f \nabla \psi),  \quad  x\in  \Omega, \; t>0 \\
  &\partial_n f+ \partial_n \psi f=0, \quad x\in \partial\Omega,\\
  & f(0,x)=f_0(x),\quad x\in \Omega.
  \end{align} 
 \end{subequations}
 We observe that the FP equation (\ref{fp}a) becomes the PNP system (\ref{mc}a) with $m=1$ and $q_1=1$, if the potential $\psi$ is determined by the Poisson equation (\ref{mc}b) instead of externally given. Motivated by this observation, we will design and analyze a DDG scheme for the PNP system that preserves the positivity of the solution $c_i$.

